Learning From Free-Text Human Feedback -- Collect New Datasets Or Extend Existing Ones?

Learning from free-text human feedback is essential for dialog systems, but annotated data is scarce and usually covers only a small fraction of error types known in conversational AI. Instead of collecting and annotating new datasets from scratch, recent advances in synthetic dialog generation could be used to augment existing dialog datasets with the necessary annotations. However, to assess the feasibility of such an effort, it is important to know the types and frequency of free-text human feedback included in these datasets. In this work, we investigate this question for a variety of commonly used dialog datasets, including MultiWoZ, SGD, BABI, PersonaChat, Wizards-of-Wikipedia, and the human-bot split of the Self-Feeding Chatbot. Using our observations, we derive new taxonomies for the annotation of free-text human feedback in dialogs and investigate the impact of including such data in response generation for three SOTA language generation models, including GPT-2, LLAMA, and Flan-T5. Our findings provide new insights into the composition of the datasets examined, including error types, user response types, and the relations between them.

==> acl_sty_ <==
% This is the LaTex style file for *ACL.
% The official sources can be found at
%
%     https://github.com/acl-org/acl-style-files/
%
% This package is activated by adding
%
%    \usepackage{acl}
%
% to your LaTeX file. When submitting your paper for review, add the "review" option:
%
%    \usepackage[review]{acl}

\newif\ifacl@finalcopy
\DeclareOption{final}{\acl@finalcopytrue}
\DeclareOption{review}{\acl@finalcopyfalse}
\ExecuteOptions{final} % final copy is the default

% include hyperref, unless user specifies nohyperref option like this:
% \usepackage[nohyperref]{acl}
\newif\ifacl@hyperref
\DeclareOption{hyperref}{\acl@hyperreftrue}
\DeclareOption{nohyperref}{\acl@hyperreffalse}
\ExecuteOptions{hyperref} % default is to use hyperref
\ProcessOptions\relax

\typeout{Conference Style for ACL}

\usepackage{xcolor}	

\ifacl@finalcopy
  % Hack to ignore these commands, which review mode puts into the .aux file.
  \newcommand{\@LN@col}[1]{}
  \newcommand{\@LN}[2]{}
\else
  % Add draft line numbering via the lineno package
  % https://texblog.org/2012/02/08/adding-line-numbers-to-documents/
  \usepackage[switch,mathlines]{lineno}

  % Line numbers in gray Helvetica 8pt
  \font\aclhv = phvb at 8pt
  \renewcommand\linenumberfont{\aclhv\color{lightgray}}

  % Zero-fill line numbers
  % NUMBER with left flushed zeros  \fillzeros[<WIDTH>]<NUMBER>
  \newcount\cv@tmpc@ \newcount\cv@tmpc
  \def\fillzeros[#1]#2{\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi
    \cv@tmpc=1 %
    \loop\ifnum\cv@tmpc@<10 \else \divide\cv@tmpc@ by 10 \advance\cv@tmpc by 1 \fi
       \ifnum\cv@tmpc@=10\relax\cv@tmpc@=11\relax\fi \ifnum\cv@tmpc@>10 \repeat
    \ifnum#2<0\advance\cv@tmpc1\relax-\fi
    \loop\ifnum\cv@tmpc<#1\relax0\advance\cv@tmpc1\relax\fi \ifnum\cv@tmpc<#1 \repeat
    \cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi \relax\the\cv@tmpc@}%
  \renewcommand\thelinenumber{\fillzeros[3]{\arabic{linenumber}}}
  \linenumbers

  \setlength{\linenumbersep}{1.6cm}

  % Bug: An equation with $$ ... $$ isn't numbered, nor is the previous line.

  % Patch amsmath commands so that the previous line and the equation itself
  % are numbered. Bug: multline has an extra line number.
  % https://tex.stackexchange.com/questions/461186/how-to-use-lineno-with-amsmath-align
  \usepackage{etoolbox} %% <- for \pretocmd, \apptocmd and \patchcmd
  
  \newcommand*\linenomathpatch[1]{%
    \expandafter\pretocmd\csname #1\endcsname {\linenomath}{}{}%
    \expandafter\pretocmd\csname #1*\endcsname {\linenomath}{}{}%
    \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
    \expandafter\apptocmd\csname end#1*\endcsname {\endlinenomath}{}{}%
  }
  \newcommand*\linenomathpatchAMS[1]{%
    \expandafter\pretocmd\csname #1\endcsname {\linenomathAMS}{}{}%
    \expandafter\pretocmd\csname #1*\endcsname {\linenomathAMS}{}{}%
    \expandafter\apptocmd\csname end#1\endcsname {\endlinenomath}{}{}%
    \expandafter\apptocmd\csname end#1*\endcsname {\endlinenomath}{}{}%
  }
  
  %% Definition of \linenomathAMS depends on whether the mathlines option is provided
  \expandafter\ifx\linenomath\linenomathWithnumbers
    \let\linenomathAMS\linenomathWithnumbers
    %% The following line gets rid of an extra line numbers at the bottom:
    \patchcmd\linenomathAMS{\advance\postdisplaypenalty\linenopenalty}{}{}{}
  \else
    \let\linenomathAMS\linenomathNonumbers
  \fi

  \AtBeginDocument{%
    \linenomathpatch{equation}%
    \linenomathpatchAMS{gather}%
    \linenomathpatchAMS{multline}%
    \linenomathpatchAMS{align}%
    \linenomathpatchAMS{alignat}%
    \linenomathpatchAMS{flalign}%
  }
\fi

\iffalse
\PassOptionsToPackage{
  a4paper,
  top=2.21573cm,left=2.54cm,
  textheight=24.7cm,textwidth=16.0cm,
  headheight=0.17573cm,headsep=0cm
}{geometry}
\fi
\PassOptionsToPackage{a4paper,margin=2.5cm}{geometry}
\RequirePackage{geometry}

\setlength\columnsep{0.6cm}  
\newlength\titlebox 
\setlength\titlebox{5cm}

\twocolumn \sloppy

% We're never going to need a table of contents, so just flush it to
% save space --- suggested by drstrip@sandia-2
\def\addcontentsline#1#2#3{}

\ifacl@finalcopy
    \thispagestyle{empty}        
    \pagestyle{empty}
\else
    \pagenumbering{arabic}
\fi

%% Title and Authors %%

\newcommand{\Thanks}[1]{\thanks{\ #1}}

\newcommand\outauthor{
    \begin{tabular}[t]{c}
    \ifacl@finalcopy
	     \bf\@author
	\else 
		% Avoiding common accidental de-anonymization issue. --MM
        \bf Anonymous ACL submission
	\fi
    \end{tabular}}

% Mostly taken from deproc.
\AtBeginDocument{
\def\maketitle{\par
 \begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox to 0pt{$^{\@thefnmark}$\hss}}
   \twocolumn[\@maketitle] \@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}
\def\@maketitle{\vbox to \titlebox{\hsize\textwidth
 \linewidth\hsize \vskip 0.125in minus 0.125in \centering
 {\Large\bf \@title \par} \vskip 0.2in plus 1fil minus 0.1in
 {\def\and{\unskip\enspace{\rm and}\enspace}%
  \def\And{\end{tabular}\hss \egroup \hskip 1in plus 2fil 
           \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf}%
  \def\AND{\end{tabular}\hss\egroup \hfil\hfil\egroup
          \vskip 0.25in plus 1fil minus 0.125in
           \hbox to \linewidth\bgroup\large \hfil\hfil
             \hbox to 0pt\bgroup\hss \begin{tabular}[t]{c}\bf}
  \hbox to \linewidth\bgroup\large \hfil\hfil
    \hbox to 0pt\bgroup\hss 
	\outauthor
   \hss\egroup
    \hfil\hfil\egroup}
  \vskip 0.3in plus 2fil minus 0.1in
}}
}

% margins and font size for abstract
\renewenvironment{abstract}%
		 {\centerline{\large\bf Abstract}%
		  \begin{list}{}%
		     {\setlength{\rightmargin}{0.6cm}%
		      \setlength{\leftmargin}{0.6cm}}%
		   \item[]\ignorespaces%
		   \@setsize\normalsize{12pt}\xpt\@xpt
		   }%
		 {\unskip\end{list}}
  
%\renewenvironment{abstract}{\centerline{\large\bf  
% Abstract}\vspace{0.5ex}\begin{quote}}{\par\end{quote}\vskip 1ex}

% Resizing figure and table captions - SL
% Support for interacting with the caption, subfigure, and subcaption packages - SL
\RequirePackage{caption}
\DeclareCaptionFont{10pt}{\fontsize{10pt}{12pt}\selectfont}
\captionsetup{font=10pt}

\RequirePackage{natbib}
% for citation commands in the .tex, authors can use:
% \citep, \citet, and \citeyearpar for compatibility with natbib, or
% \cite, \newcite, and \shortcite for compatibility with older ACL .sty files
\renewcommand\cite{\citep}	% to get "(Author Year)" with natbib    
\newcommand\shortcite{\citeyearpar}% to get "(Year)" with natbib    
\newcommand\newcite{\citet}	% to get "Author (Year)" with natbib

\bibliographystyle{acl_natbib}

% Bibliography

% Don't put a label in the bibliography at all.  Just use the unlabeled format
% instead.
\def\thebibliography#1{\vskip\parskip%
\vskip\baselineskip%
\def\baselinestretch{1}%
\ifx\@currsize\normalsize\@normalsize\else\@currsize\fi%
\vskip-\parskip%
\vskip-\baselineskip%
\section*{References\@mkboth
 {References}{References}}\list
 {}{\setlength{\labelwidth}{0pt}\setlength{\leftmargin}{\parindent}
 \setlength{\itemindent}{-\parindent}}
 \def\newblock{\hskip .11em plus .33em minus -.07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist


% Allow for a bibliography of sources of attested examples
\def\thesourcebibliography#1{\vskip\parskip%
\vskip\baselineskip%
\def\baselinestretch{1}%
\ifx\@currsize\normalsize\@normalsize\else\@currsize\fi%
\vskip-\parskip%
\vskip-\baselineskip%
\section*{Sources of Attested Examples\@mkboth
 {Sources of Attested Examples}{Sources of Attested Examples}}\list
 {}{\setlength{\labelwidth}{0pt}\setlength{\leftmargin}{\parindent}
 \setlength{\itemindent}{-\parindent}}
 \def\newblock{\hskip .11em plus .33em minus -.07em}
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthesourcebibliography=\endlist

% sections with less space
\def\section{\@startsection {section}{1}{\z@}{-2.0ex plus
    -0.5ex minus -.2ex}{1.5ex plus 0.3ex minus .2ex}{\large\bf\raggedright}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-1.8ex plus
    -0.5ex minus -.2ex}{0.8ex plus .2ex}{\normalsize\bf\raggedright}}
%% changed by KO to - values to get the initial parindent right
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-1.5ex plus
   -0.5ex minus -.2ex}{0.5ex plus .2ex}{\normalsize\bf\raggedright}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{1.5ex plus
   0.5ex minus .2ex}{-1em}{\normalsize\bf}}
\def\subparagraph{\@startsection{subparagraph}{5}{\parindent}{1.5ex plus
   0.5ex minus .2ex}{-1em}{\normalsize\bf}}

% Footnotes
\footnotesep 6.65pt %
\skip\footins 9pt plus 4pt minus 2pt
\def\footnoterule{\kern-3pt \hrule width 5pc \kern 2.6pt }
\setcounter{footnote}{0}

% Lists and paragraphs
\parindent 1em
\topsep 4pt plus 1pt minus 2pt
\partopsep 1pt plus 0.5pt minus 0.5pt
\itemsep 2pt plus 1pt minus 0.5pt
\parsep 2pt plus 1pt minus 0.5pt

\leftmargin 2em \leftmargini\leftmargin \leftmarginii 2em
\leftmarginiii 1.5em \leftmarginiv 1.0em \leftmarginv .5em \leftmarginvi .5em
\labelwidth\leftmargini\advance\labelwidth-\labelsep \labelsep 5pt

\def\@listi{\leftmargin\leftmargini}
\def\@listii{\leftmargin\leftmarginii
   \labelwidth\leftmarginii\advance\labelwidth-\labelsep
   \topsep 2pt plus 1pt minus 0.5pt
   \parsep 1pt plus 0.5pt minus 0.5pt
   \itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
    \labelwidth\leftmarginiii\advance\labelwidth-\labelsep
    \topsep 1pt plus 0.5pt minus 0.5pt 
    \parsep \z@ \partopsep 0.5pt plus 0pt minus 0.5pt
    \itemsep \topsep}
\def\@listiv{\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv\advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
     \labelwidth\leftmarginv\advance\labelwidth-\labelsep}
\def\@listvi{\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi\advance\labelwidth-\labelsep}

\abovedisplayskip 7pt plus2pt minus5pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip  0pt plus3pt%   
\belowdisplayshortskip  4pt plus3pt minus3pt%

% Less leading in most fonts (due to the narrow columns)
% The choices were between 1-pt and 1.5-pt leading
\def\@normalsize{\@setsize\normalsize{11pt}\xpt\@xpt}
\def\small{\@setsize\small{10pt}\ixpt\@ixpt}
\def\footnotesize{\@setsize\footnotesize{10pt}\ixpt\@ixpt}
\def\scriptsize{\@setsize\scriptsize{8pt}\viipt\@viipt}
\def\tiny{\@setsize\tiny{7pt}\vipt\@vipt}
\def\large{\@setsize\large{14pt}\xiipt\@xiipt}
\def\Large{\@setsize\Large{16pt}\xivpt\@xivpt}
\def\LARGE{\@setsize\LARGE{20pt}\xviipt\@xviipt}
\def\huge{\@setsize\huge{23pt}\xxpt\@xxpt}
\def\Huge{\@setsize\Huge{28pt}\xxvpt\@xxvpt}

% The hyperref manual (section 9) says hyperref should be loaded after natbib
\ifacl@hyperref
  \PassOptionsToPackage{breaklinks}{hyperref}
  \RequirePackage{hyperref}
  % make links dark blue
  \definecolor{darkblue}{rgb}{0, 0, 0.5}
  \hypersetup{colorlinks=true, citecolor=darkblue, linkcolor=darkblue, urlcolor=darkblue}
\else
  % This definition is used if the hyperref package is not loaded.
  % It provides a backup, no-op definiton of \href.
  % This is necessary because \href command is used in the acl_natbib.bst file.
  \def\href#1#2{{#2}}
  \usepackage{url}
\fi


==> in_depth_analysis/discussion_tfd.tex <==
Combining the findings from Tables \ref{tab:potential_errors}, \ref{tab:effectiveness}, and \ref{tab:user_reactions}, we can conclude that dialogs selected by TFD contain more error situations compared to those selected randomly. Furtheremore, the analysis of user responses annotated in random subsets (Table~\ref{tab:user_reactions}) shows that TFD seldom fails to identify relevant user responses such as UR2, UR3, or UR5 (as described in Section~\ref{sec:user_reaction_taxonomy}). However, in the rare instances where TFD misses such responses, it is due to the absence of the corresponding feedback-indicating phrases in our set of feedback-indicating sentences (Section~\ref{sec:user_reactions}).

We find TFD to be a valuable semi-automatic baseline for identifying textual user feedback in dialogs. To improve the effectiveness in future work, \sout{we suggest investigating the impact of considering more context, e.g., the dialog history or at least the previous system utterance}, we suggest to finetune the underlying sentence-transformer on EURTAD. It might also be interesting to increase the number and variety of feedback-indicating sentences. Another valuable approach might be to add a classification layer on top. This way, TFD could also be enabled to directly annotate system utterances for containing errors and user utterances for potentially containing textual feedback.

==> in_depth_analysis/taxonomy_improvements.tex <==
Based on our findings from Section~\ref{sec:crowd_workers}, we propose a condensed version of the integrated error taxonomy \citet{higashinaka2021integrated} for the purpose of free-form text feedback detection. Table~\ref{tab:improved_taxonomy} shows this new taxonomy.

\begin{table}[ht]
  \centering
  \input{tables/improved_taxonomy.tex}
\caption{Improved Taxonomy.}
\label{tab:improved_taxonomy}
  \end{table}

We ignore the utterance-level error types from the original taxonomy, i.e., \textit{uninterpretable} (I1), \textit{grammatical error} (I2) and \textit{semantic error} (I3), as we never observe them at all in our analysis. Furthermore, we ignore \textit{lack of information} (I12), a context-level error type very similar to I2, and \textit{ignore proposal} (I7), a response-level error type very similar to I6 (E2 in Table~\ref{tab:improved_taxonomy}), for the same reasons. This does not mean that these error types are in general irrelevant. They just do not cause free-form text feedback.
Next, we merge \textit{ignore greeting} (I8) with \textit{lack of sociality} (I16, now E9), as the latter implies the first one. We only rarely observe \textit{contradiction} (I14), and only as a result of \textit{lack of common sense} (I17, now E10) or \textit{factually incorrect} (E5) errors, which is why we ignore it as an error type on its own. E5 is a new error types that replaces \textit{wrong information} (I4) by extending its original definition for taking also factual incorrect knowledge into account. We also merge \textit{repetition} (I15) and \textit{self-contradiction} (I13) to what we call \textit{conversationality} (E7), as we observe both error types rarely, and if, only in situations that suggest that the system has lost the thread.
We also observe cases of (obviously) incorrectly conveyed errors in task-oriented dialogs that were not covered by the original taxonomy. For such cases, we introduce \textit{slot error} (E7). Table~\ref{tab:improved_iaa} shows the improvements in inter-annotator agreement when using this new taxonomy.

\begin{table}[ht]
  \centering
  \input{tables/improved_inter_annotator.tex}
\caption{Inter-Annotator-Agreement when using the condensed taxonomy. It improves the agreement on the conspicuous dataset.}
\label{tab:improved_iaa}
  \end{table}

Using this new taxonomy mostly improves the agreement for MWoZ~\citep{budzianowski2018multiwoz}, PC~\citep{zhang2018personalizing}, and SFC~\citep{hancock2019learning}. It has only little or no effect on the other datasets (the changed error types are not or only rarely observed in these datasets).


==> tables/class_distribution_random_subsets.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{crrrrrrrrrrrrrrrrrr}
\multicolumn{1}{l}{} &
  \multicolumn{9}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Task-\\ Oriented\end{tabular}}} &
  \multicolumn{6}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Domain\end{tabular}}} &
  \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Know.-\\ Grounded\end{tabular}}} \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}MWoZ\\ (HH)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}SGD\\ (HH)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}BABI\\ (HB)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}PC\\ (HH)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}SFC\\ (HB)\end{tabular}} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}WoW\\ (HH)\end{tabular}} \\ \hline
\multicolumn{1}{c|}{\textbf{Annotator}} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c}{A3} \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ignore\\ Question (E1)\end{tabular}}} &
  - &
  1 &
  \multicolumn{1}{r|}{1} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  \multicolumn{1}{r|}{3} &
  5 &
  2 &
  \multicolumn{1}{r|}{5} &
  - &
  1 &
  2 \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ignore\\ Request (E2)\end{tabular}}} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  2 &
  3 &
  \multicolumn{1}{r|}{2} &
  - &
  - &
  - \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Ignore\\ Expect. (E3)\end{tabular}}} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  - \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Slot\\ Error (E4)\end{tabular}}} &
  - &
  1 &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  \multicolumn{1}{r|}{1} &
  - &
  2 &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  - \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Factually\\ Incorrect (E5)\end{tabular}}} &
  - &
  1 &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  4 &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  - \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Topic Trans.\\ Error (E6)\end{tabular}}} &
  - &
  - &
  \multicolumn{1}{r|}{1} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{6} &
  16 &
  14 &
  \multicolumn{1}{r|}{11} &
  - &
  - &
  1 \\ \hline
\multicolumn{1}{c|}{\textbf{Convers. (E7)}} &
  - &
  - &
  \multicolumn{1}{r|}{1} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  \multicolumn{1}{r|}{1} &
  - &
  - &
  \multicolumn{1}{r|}{2} &
  1 &
  - &
  1 \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Unclear\\ Intention (E8)\end{tabular}}} &
  - &
  12 &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  12 &
  - \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Lack of \\ Sociality (E9)\end{tabular}}} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  1 &
  \multicolumn{1}{r|}{2} &
  - &
  2 &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  - \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Lack of \\ Com. Sense \\ (E10)\end{tabular}}} &
  - &
  - &
  \multicolumn{1}{r|}{1} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  1 &
  1 &
  \multicolumn{1}{r|}{1} &
  - &
  - &
  \multicolumn{1}{r|}{-} &
  1 &
  - &
  1
\end{tabular}
}

==> tables/class_distribution_user_responses_random_subsets.tex <==
\resizebox*{\linewidth}{!}{
\begin{tabular}{crrrrrrrrrrrrrrrrrr}
\multicolumn{1}{l}{} &
  \multicolumn{9}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Task-\\ Oriented\end{tabular}}} &
  \multicolumn{6}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Domain\end{tabular}}} &
  \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Know.-\\ Grounded\end{tabular}}} \\ \hline
\multicolumn{1}{l|}{} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}MWoZ\\ (HH)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}SGD\\ (HH)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}BABI\\ (HB)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}PC\\ (HH)\end{tabular}} &
  \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}SFC\\ (HB)\end{tabular}} &
  \multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}}WoW\\ (HH)\end{tabular}} \\ \hline
\multicolumn{1}{c|}{\textbf{Annotator}} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c|}{A3} &
  \multicolumn{1}{c}{A1} &
  \multicolumn{1}{c}{A2} &
  \multicolumn{1}{c}{A3} \\ \hline
\multicolumn{1}{c|}{\textbf{UR1}} &
   &
  6 &
  \multicolumn{1}{r|}{1} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
  2 &
  \multicolumn{1}{r|}{} &
   &
   &
  \multicolumn{1}{r|}{13} &
  16 &
  15 &
  \multicolumn{1}{r|}{13} &
  1 &
  10 &
  3 \\ \hline
\multicolumn{1}{c|}{\textbf{UR2}} &
   &
  7 &
  \multicolumn{1}{r|}{-} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
  2 &
  \multicolumn{1}{r|}{} &
   &
   &
  \multicolumn{1}{r|}{1} &
   &
  1 &
  \multicolumn{1}{r|}{} &
   &
   &
   \\ \hline
\multicolumn{1}{c|}{\textbf{UR3}} &
   &
   &
  \multicolumn{1}{r|}{2} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
  1 &
  \multicolumn{1}{r|}{} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
  1 &
  \multicolumn{1}{r|}{} &
   &
  1 &
  2 \\ \hline
\multicolumn{1}{c|}{\textbf{UR4}} &
   &
  2 &
  \multicolumn{1}{r|}{1} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
   &
  \multicolumn{1}{r|}{} &
  1 &
  4 &
  \multicolumn{1}{r|}{} &
  2 &
  3 &
  \multicolumn{1}{r|}{2} &
  1 &
   &
   \\ \hline
\multicolumn{1}{c|}{\textbf{UR5}} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
   &
  \multicolumn{1}{r|}{} &
   &
  1 &
  \multicolumn{1}{r|}{} &
  5 &
  4 &
  \multicolumn{1}{r|}{5} &
   &
  4 &
  
\end{tabular}}

==> tables/error_types_user_reactions.tex <==
\resizebox*{\linewidth}{!}{\begin{tabular}{cc|rrrr|rr}
\multirow{2}{*}{\textbf{}}        & \multicolumn{1}{l|}{}        & \multicolumn{4}{c|}{\textbf{Human-Human}} & \multicolumn{2}{c}{\textbf{Human-Bot}} \\ \cline{3-8} 
 &
  \multicolumn{1}{l|}{} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}MWoZ\\ (TO)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}SGD\\ (TO)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}WoW \\ (KG)\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}PC\\ (OW)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}BABI\\ (TO)\end{tabular}}} &
  \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}SFC\\ (OW)\end{tabular}}} \\ \hline
\multicolumn{1}{c|}{\textbf{I9}}  & \multirow{2}{*}{\textbf{B1}} &             &            &            &   & 1                 &                    \\
\multicolumn{1}{c|}{\textbf{I11}} &                              &             &            &            &   &                   & 3                  \\ \hline
\multicolumn{1}{c|}{\textbf{I5}}  & \multirow{3}{*}{\textbf{B2}} &             &            &            &   & 1                 &                    \\
\multicolumn{1}{c|}{\textbf{I6}}  &                              & \textbf{2}  &            &            &   &                   &                    \\
\multicolumn{1}{c|}{\textbf{I9}}  &                              &             & \textbf{1} &            &   &                   &                    \\ \hline
\multicolumn{1}{c|}{\textbf{I4}}  & \multirow{3}{*}{\textbf{B3}} &             &            & \textbf{5} &   &                   &                    \\
\multicolumn{1}{c|}{\textbf{I5}}  &                              &             &            &            &   &                   & 2                  \\
\multicolumn{1}{c|}{\textbf{I6}}  &                              & 1           &            &            &   &                   &                    \\ \hline
\multicolumn{1}{c|}{\textbf{I4}}  & \multirow{6}{*}{\textbf{B4}} &             &            &            &   &                   & 1                  \\
\multicolumn{1}{c|}{\textbf{I5}}  &                              &             & \textbf{}  &            &   & \textbf{}         & 16                 \\
\multicolumn{1}{c|}{\textbf{I6}}  &                              &             &            &            &   &                   & 1                  \\
\multicolumn{1}{c|}{\textbf{I9}}  &                              & 1           &            & 1          &   &                   &                    \\
\multicolumn{1}{c|}{\textbf{I11}} &                              &             &            &            & 1 &                   & 15                 \\
\multicolumn{1}{c|}{\textbf{I16}} &                              &             &            &            &   &                   & 1                  \\ \hline
\multicolumn{1}{c|}{\textbf{I4}}  & \multirow{5}{*}{\textbf{B5}} &             &            & 4          &   &                   & 1                  \\
\multicolumn{1}{c|}{\textbf{I5}}  &                              & 1           &            &            & 1 &                   & \textbf{32}        \\
\multicolumn{1}{c|}{\textbf{I9}}  &                              &             &            &            &   &                   & 2                  \\
\multicolumn{1}{c|}{\textbf{I11}} &                              &             &            & 4          &   &                   & 16                 \\
\multicolumn{1}{c|}{\textbf{I16}} &                              &             &            &            & 2 &                   &                   
\end{tabular}}

==> tables/potential_errors_sentence.tex <==
\resizebox*{\linewidth}{!}{\begin{tabular}{ccccccc}
\multicolumn{1}{l}{} &
  \multicolumn{3}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Task-\\ Oriented\end{tabular}}} &
  \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Open-\\ Domain\end{tabular}}} &
  \textbf{\begin{tabular}[c]{@{}c@{}}Know.-\\ Grounded\end{tabular}} \\ \hline
\multicolumn{1}{c|}{\textbf{Dataset}} &
  \begin{tabular}[c]{@{}c@{}}MWoZ\\ (HH)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}SGD\\ (HH)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}BABI\\ (HB)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}PC\\ (HH)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}SFC\\ (HB)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}WoW\\ (HH)\end{tabular} \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\#Sentences\\ (Before)\end{tabular}}} &
  103,029 &
  296,808 &
  \multicolumn{1}{c|}{192,485} &
  251,985 &
  \multicolumn{1}{c|}{190,691} &
  165,750 \\ \hline
\multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\#Sentences\\ (After)\end{tabular}}} &
  \begin{tabular}[c]{@{}c@{}}16,545\\ (16.0\%)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}19,033\\ (6.4\%)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}26,939\\ (14.0\%)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}1,474\\ (0.0\%)\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}25,711\\ (13.5\%)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}2,358\\ (1.4\%)\end{tabular}
\end{tabular}}
